PIDT: Physics-Informed Digital Twin for Optical Fiber Parameter Estimation

We propose physics-informed digital twin (PIDT): a fiber parameter estimation approach that combines a parameterized split-step method with a physics-informed loss. PIDT improves accuracy and convergence speed with lower complexity compared to previous neural operators.

==> copy/copy.tex <==
In optical fiber channels, signal propagation is governed by the NLSE, which captures linear and nonlinear impairments such as attenuation, group velocity dispersion (GVD), and self-phase modulation (SPM)
\begin{equation}\label{eq:eq1} \frac{\partial s(z,t)}{\partial z}=-\frac{\alpha}{2} s(z,t)-\frac{\mathrm{j} \beta_2}{2} \frac{\partial^2 s(z,t)}{\partial t^2}+\mathrm{j}  \gamma|s(z,t)|^2 s(z,t), \end{equation} where $s(z,t) = u(z,t) + \mathrm{j} v(z,t)$ is the complex optical baseband signal at space-time location $(z,t)$ in the optical fiber, and $\alpha$, $\beta_2$, $\gamma$ are the attenuation, GVD, and nonlinear coefficients. 

The physics-based model follows the structure of the split-step Fourier method (SSFM), which approximates the solution of the NLSE as
\begin{equation}\label{eq:eq2}
\hat{\underline{s}}^{(m)} = \sigma_m\!\big(D_m\,\hat{\underline{s}}^{(m-1)}\big), \qquad m=1,\ldots,M,
\end{equation}
where $\hat{\underline{s}}^{(m)}=[\,\hat{s}(z_m,t_1),\ldots,\, \hat{s}(z_m, t_n),\ldots,\hat{s}(z_m,t_{N})\,]^{\top}\in\mathbb{C}^{N}$ denotes the approximated signal at distance $z_m=m\Delta z$. Here, the hat symbol $\hat{(\cdot)}$ indicates a predicted or approximated signal, which is different from the ground-truth signal, and $t_n=n\Delta t$ denotes sampling period $\Delta t=T/N$, $N$ is the number of time samples, and $M$ is the number of SSFM segments with step size $\Delta z=L/M$ over the total length $L$ of fiber. For a uniform step size, the linear and nonlinear sub-steps are given by $D_m = \mathbf{F}^{-1}\,\operatorname{diag}\!\left(\exp\!\left[\Big(-\tfrac{\alpha}{2} + \mathrm{j}\tfrac{\beta_2}{2}\omega_k^{2}\Big)\Delta z\right]\right)\mathbf{F}$, and $
\sigma_m(x) = x\,\exp\!\big(\mathrm{j}\gamma\,\Delta z\,|x|^{2}\big)$,
where $\mathbf{F}$ and $\mathbf{F}^{-1}$ denote the discrete Fourier transform (DFT) and its inverse (IDFT), respectively, and $\omega_k$ is the $k$-th DFT angular frequency. By passing the transmitted signal $\underline{s}^{(0)}$ through the $D_m$ and $\sigma_m$ repeatly for all segments $m=1,2,\ldots,M$, we can get the numerical close-form solution for Eq.~\eqref{eq:eq1}. As an additional benefit, fiber-related parameters can be directly extracted during the training of the physics-based model. Both the forward system model~\cite{sasai2023performance} and the inverse system model \cite{sasai2021digital} can be employed for parameter estimation, and we adopt the forward system model in this work. The design and training procedure of the physics-based model is illustrated in Fig.~\ref{fig:bg1}. For each segment, a pair of segment-wise parameters is defined, so the whole parameter set for physics-based model denoted as ${\theta}_{\text{d}}=\{{\beta'_2}^{(m)},\, {\gamma'}^{(m)}\}^{M}_{m=1}$, where the prime indicates tunable parameters. The parameters $\theta_\text{d}$ are estimated by minimizing the MSE-based input-output signal pairs loss (IO loss) $L_\text{io}(\theta_\text{d})=\frac{1}{N} \sum|\hat{\underline{s}}^{(M)}-\underline{s}^{(M)}|^2$ between the reference received signals $\underline{s}^{(M)}$ and predicted one $\hat{\underline{s}}^{(M)}$. Different from black-box neural networks, the physics-based model contains only $2M$ physically interpretable parameters, which enables it to learn to predict the received signals both quickly and accurately. However, training solely with IO loss may cause the estimated parameters $\theta_\text{d}$ to lack physical consistency. This limitation motivates us to physics-informed loss, which has been utilized in PINO for optical fiber parameter estimation~\cite{songPhysicsInformedNeuralOperatorbased2023}.

The PINO structure designed for optical fiber systems~\cite{songPhysicsInformedNeuralOperator2022, songPhysicsInformedNeuralOperatorbased2023} aims to learn a neural operator that approximates the NLSE, mapping transmitted complex signals $s(0,t)$ as an initial condition to their solutions $s(z,t)$ at the corresponding space-time coordinates $(z,t)$ in the solver domain, with the operator represented as $G_{\theta_\text{g}}$, parameterized by the trainable set $\theta_\text{g}$. As illustrated in Fig.~\ref{fig:bg2}, the operator consists of a trunk net and a branch net, with parameters $\theta_\text{g}=\left\{\left\{\theta_i^{(l)},\vartheta_i^{(l)}\right\}_{i=1}^Q\right\}_{l=1}^J$, where $\bigl\{\{\theta_i^{(l)}\}_{i=1}^Q\bigr\}_{l=1}^J$ denotes the parameters of the branch net with $Q$ neurons per layer and $J$ hidden layers, and $\bigl\{\{\vartheta_i^{(l)}\}_{i=1}^Q\bigr\}_{l=1}^J$ denotes the parameters of the trunk net. The trunk net encodes the input coordinates $(z,t)$ into embeddings $[f_1,\ldots,f_q]$ of feature length $q$. The branch net processes the transmitted complex signal as the initial condition. Specifically, the complex input signals is represented by concatenating its real and imaginary parts $[u(0,t_1),\ldots,u(0,t_N),v(0,t_1),\ldots,v(0,t_N)]^{\mathsf T}$, where the first half corresponds to the real part and the second half to the imaginary part. The branch net then outputs the corresponding embeddings $[k^{\text{R}}_1,\ldots,k^{\text{R}}_q, k^{\text{I}}_1,\ldots,k^{\text{I}}_q]$, where $k^{\text{R}}$ and $k^{\text{I}}$ represent the embeddings of the real and imaginary components, respectively. By merging the embeddings from the branch and trunk nets via dot product $\hat{s}(z,t)=\sum_{i=1}^q k^{\text{R}}_i f_i + \mathrm{j}\sum_{i=1}^q k^{\text{I}}_i f_i$, the predicted signal value $\hat{s}(z,t)$ at a given space–time coordinate is obtained. Since the learnable operator in a PINO is a black-box neural network, the fiber parameters cannot be directly extracted from $G_{\theta_\text{g}}$. However, these fiber parameters are explicitly included in the physics-informed loss used during PINO training, which can be expressed as
\begin{equation}
\begin{aligned}
& R(z,t)=\frac{\partial \hat{s}(z,t)}{\partial z}+\frac{\alpha}{2} \hat{s}(z,t)+i \frac{\beta'_2}{2} \frac{\partial^2 \hat{s}(z,t)}{\partial t^2}-i \gamma' \hat{s}(z,t)|\hat{s}(z,t)|^2 \\
& L_\text{p}(\theta_\text{g},\theta_\text{p})=\frac{1}{|X|} \sum_{(z,t) \in X} |{R}(z,t)|
\end{aligned},
\end{equation}
where $R(z,t)$ is the PDE residual that derived from the NLSE, and $L_\text{p}(\theta_\text{g},\theta_\text{p})$ is the physics-informed loss that drives the residual toward zero over all sampled coordinates in the set $X$, whose size is denoted by $|X|$, by updating the parameter sets $\theta_\text{g}$ and $\theta_\text{p}$. Here we adopt the $\ell_1$ loss for the residual instead of the conventional $\ell_2$ loss, as the $\ell_1$ loss is less sensitive to outliers and thus improves robustness when the predicted signals contain local inaccuracies or noise~\cite{boyd2004convex}. Here, ${\theta}_{\text{p}}=\{\beta'_2,\, \gamma'\}$ represents the trainable fiber parameters included in the residual, parameters selection is guided by~\cite{songPhysicsInformedNeuralOperatorbased2023}. By minimizing the $L_\text{p}$, PINO learns the operator $G_{\theta_\text{g}}$ to behave consistently with the NLSE described in $R(z,t)$ for all input coordinates in solver domain, while simultaneously estimating the parameter set $\theta_{\text{p}}$ so that the NLSE aligns with the predicted signal $\hat{s}(z,t)$. However, the fiber parameters cannot be reliably estimated using only $L_\text{p}(\theta_\text{g},\theta_\text{p})$, because incorrect $\theta_\text{p}$ may mislead the training of $G_{\theta_\text{g}}$, and an NLSE with incorrect parameters can still match an incorrect prediction from $G_{\theta_\text{g}}$. Therefore, training PINO solely with $L_\text{p}$ is insufficient. As shown in Fig.~\ref{fig:bg2}, the PINO-based parameter estimator is trained using three different losses~\cite{songPhysicsInformedNeuralOperatorbased2023}: the physics-informed loss $L_\text{p}(\theta_\text{g},\theta_\text{p})$, the initial condition loss $L_\text{ic}(\theta_\text{g})$, and the IO loss $L_\text{io}(\theta_\text{g})$. The physics-informed loss encourages the operator to satisfy the NLSE residual $R(z,t)$, the IO loss ensures that the predicted received signals $\hat{\mathbf{s}}^{(M)}$ match the ground truth, and the initial condition loss enforces the correct initial conditions for the operator. These three losses are combined by a weighted combination $L(\theta_\text{g},\theta_\text{p}) = \lambda_\text{io} L_\text{io}(\theta_\text{g}) + \lambda_\text{ic} L_\text{ic}(\theta_\text{g}) + \lambda_\text{p} L_\text{p}(\theta_\text{g},\theta_\text{p}),$ and a loss-balancing scheme in~\cite{wang2023expert} is adopted for jointly training. After training, the fiber parameters can be directly extracted from the learned set $\theta_\text{p}$. However, the estimation accuracy is highly sensitive to the network design, and achieving good performance often requires complex hyperparameter tuning, which reduces efficiency.



% Proposed
As introduced earlier, the physics-based model has stronger physics interpretability, meaning that its convergence is typically faster and that fiber parameters can be directly extracted from the trained model. However, the absence of explicit physical constraints during training may lead to physics-inconsistent estimates of the fiber parameters. 

In the PINO framework, neural networks are used to learn the operator itself, making it impossible to extract fiber parameters from the learned model directly. By introducing a parameterized physics-informed loss, one can estimate fiber parameters from the neural operator; however, this approach requires careful and often laborious hyperparameter tuning as well as complex neural network architectures to achieve accurate parameter estimation.

The main idea of this paper is to propose a new method, termed PIDT, that combines the advantages of both physics-based models and physics-informed losses by replacing the neural network structure in PINO with a physics-based model. However, a direct plug-and-play substitution is not feasible for PIDT because of the mismatch between the interfaces of the neural operator and the physics-based model. Specifically, the input of the physics-based model is the transmitted signal, and its output is the predicted received signal. In contrast, the inputs of the neural operator in PINO consist of the initial condition together with sampled coordinates from the solution domain, and the output is the signal value of the initial condition at the specified coordinate. To bridge this gap, we propose a modified digital twin model, which builds on the physics-based model and incorporates interpolation to align the interfaces, as illustrated in Fig.~\ref{fig:bg3}.


\section{Numerical Results} To evaluate the proposed PIDT method, we compare its performance against both the PINO-based estimator and the physics-based model-based estimator. The transmission setting follows~\cite{songPhysicsInformedNeuralOperator2022}: 16-QAM modulation at a symbol rate of 14~Gbaud with root-raised-cosine (RRC) pulses (roll-off factor 0.1). The discretized transmitted signal $\underline{s}^{(0)}$ is generated with $N$ symbols, oversampling factor $\rho=2$, and launch power $P_0=0$~dBm. Unless otherwise specified, we consider $N=512$ for simulations. For the optical link, a single-span system of length $L=80$~km is simulated. Amplified spontaneous emission (ASE) noise is added at the end of the span with $\text{SNR}=20$~dB. To emulate the true link, the SSFM is performed with step size $\Delta z=200$~m, and its outputs are treated as ground-truth received signals for both training and evaluation. To ensure effective training, the normalized NLSE formulation is adopted, following the frame transformation in~\cite{zangPrincipleDrivenFiberTransmission2022}. Fiber attenuation is neglected in the simulations, as the focus is on estimating $\beta_2$ and $\gamma$. For the trainable parameters in PIDT, scaling factors are applied to adjust both the constant fiber parameters in the loss and the segment-wise parameters in the digital twin to a comparable magnitude for effective training, similar to the strategy in~\cite{jiangPhysicsInformedNeuralNetwork2022}. To compare the PINO and PIDT, $|X|=20^4$ space–time coordinates are sampled uniformly, and 500 pairs of noise-free transmitted/received signals are collected. During training, noise is randomly generated according to $\text{SNR}=10\log_{10}(P_s/P_n)$, where $P_s$ and $P_n$ denote the signal and noise powers, respectively, and added to the received signals at the beginning of each iteration. Training is performed for $10^5$ iterations with a batch size of 20 signals and 800 coordinates. The Adam optimizer~\cite{adam2014method} is employed with an initial learning rate of $10^{-3}$, decayed by a factor of 0.9 every 5000 steps. For PINO, network structures with $Q=q\in\{200,\,600,\,1000\}$ neurons and $J=3$ hidden layers are activated by the tanh function, and parameters are randomly initialized based on~\cite{lu2021learning}. For PIDT, the number of steps is set to $M=4$, and experiments are repeated for signals with different numbers of symbols $N\in\{32,\,64,\,128,\,256,\,512\}$. The constant fiber parameters in the physics-informed loss are initialized to zero, following~\cite{jiangPhysicsInformedNeuralNetwork2022}, while the parameters in the digital twin of PIDT are also initialized to zero, consistent with~\cite{sasai2021digital}. The parameter estimation results under these settings are reported in Fig.~\ref{fig:xxx}. Here, we do a comparison between the physics-informed model and PIDT. We focus on signals with $N=512$ symbols. PIDT and the physics-based model are compared with different numbers of steps $M\in\{4,\,10\}$. Parameters in both PIDT and the physics-based model are initialized to zero, consistent with~\cite{sasai2021digital}. The optimization settings remain the same as above. The estimated parameters are compared in Fig.~\ref{fig:yyy}. An additional advantage of PIDT is that it can estimate not only segment-wise parameters from the twin model but also constant fiber parameters jointly from the physics-informed loss. Finally, we investigate the robustness of PIDT under different noise conditions with $\text{SNR}\in\{20,\,10,\,5,\,0\}$ compare with PINO. The PIDT with $M=4$ is considered, and PINO with the highest complexity. As shown in Fig.~\ref{fig:yyy}, the relative error is used to evaluate the estimated constant fiber parameters extracted from the physics-informed loss.

==> figures/copy_figures.tex <==
\newcommand{\pbm}{%
\begin{tikzpicture}
      \foreach \x in {2.7,2.9,3.1} {
        \draw[black, thick, fill=white] (\x,2.6) ellipse [x radius=0.2, y radius=0.4];
      }
      \draw[-{Latex[length=2mm]}, thick] (0.5,2.2) -- (6.9,2.2);
      \draw[thick, fill=white] (4.3+1.7*0.4,2.2) -- (4.3,2.6) -- (4.3,1.8) -- cycle;
    
      \node at (0.2, 2.3) {$\underline{s}^{(0)}$};
      \node at (7.45, 2.3) {$\underline{s}^{(M)}$};
      \node at (5, 3) {\small Optical fiber channel};

    % Physics-based model
    \draw[-{Latex[length=2mm]}, thick] (0.5,0) -- (6.9,0);

    \draw[color=RoyalBlue, fill=RoyalBlue!10, rounded corners=3pt, thick] (1,-1.2) rectangle (6,1.5); \node[align=left] at (2.5, 1.25) {\small Physics-based model};
    \draw[thick] (1.01,0) -- (2.475,0); \draw[thick] (3.75+0.775,0) -- (5.99,0);

    \foreach \x/\eq in {1.2/ ${{\beta'_2}^{(1)}, {\gamma'}^{(1)}}$, 2.475/${{\beta'_2}^{(2)}, {\gamma'}^{(2)}}$, 3.75/${{\beta'_2}^{(M-1)}, {\gamma'}^{(M-1)}}$, 5.025/${{\beta'_2}^{(M)}, {\gamma'}^{(M)}}$} {\draw[color=white, rounded corners=3pt, fill=white, thick] (\x, -1) rectangle (\x+0.775, 1); \node[rotate=90, align=center] at (\x+0.3875, 0) {\footnotesize \eq};}

    \filldraw[gray] (1.2+0.775+0.25,0) circle [radius=2pt];
    \filldraw[gray] (3.75+0.775+0.25,0) circle [radius=2pt];

    \node[rotate=90, align=center] at (1.2+1.04, 0.35) {\small $\underline{\hat{s}}^{(1)}$};
    \node[rotate=90, align=center] at (3.75+1.04, 0.55) {\small $\underline{\hat{s}}^{(M-1)}$};

    \node at (3.5,0) {\normalsize $\cdots$};

    \node at (0.2, 0) {$\underline{s}^{(0)}$};

    \draw[fill=white, thick, rounded corners=3pt](6.9, -0.4) rectangle (8, 0.25); \node at (7.45, -0.075) {\small $L_\text{o}(\theta_\text{d})$};

    % arrow from optical link
    \draw[-{Latex[length=2mm]}, thick] (7.45, 0.8) -- (7.45, 0.25);
    \node at (7.45, 1) {$\underline{s}^{(M)}$};

    \node at (6.5, 0.3) {$\hat{\underline{s}}^{(M)}$};

    % arrow from loss to model
    \draw[-{Latex[length=2mm]}, dash pattern=on 4pt off 2pt, thick] (6.9,-0.2) -- (6,-0.2);

    \node[align=left] at (7.35, -0.8) {\footnotesize Update\\  \footnotesize ${\theta}_{\text{d}}=\{ {\beta'_2}^{(m)}, {\gamma'}^{(m)} \}_{m=1}^M$};
    
\end{tikzpicture}%
}

% PINO structure
\newcommand{\pino}{
\begin{tikzpicture}
    % ---- inputs on the left ----
    \draw[thick] (0.5,-0.4) -- (1,-0.4); \node at (0.15, -0.4) {$(z,t)$};
    \draw[thick] (0.5,0.1)  -- (1,0.1);  \node at (0.15,  0.1){$\underline{s}^{(0)}$};

    % ---- PINO block (left) ----
    \draw[color=ForestGreen, fill=ForestGreen!10, rounded corners=3pt, thick]
      (1,-0.8) rectangle (4,0.8);
    \node[align=center] at (1.55, 0.55) {\small PINO};
    \draw[thick] (1.01,-0.4) -- (2,-0.4);
    \draw[thick] (1.01,0.1)  -- (2,0.1);
    \draw[thick] (2,-0.15) -- (3.99,-0.15);
    \draw[color=white, rounded corners=3pt, fill=white, thick]
      (1.2, -0.6) rectangle (3.8, 0.3);
    \node at (2.5, -0.15) {$G(\theta_\text{g})$};
    \node at (4.4, -0.45) {$\hat{s}(z,t)$};

    \filldraw[black] (0.75, 0.1) circle [radius=2pt];

    % ---- Loss block (right, horizontally placed) ----
    \draw[color=RedOrange, fill=RedOrange!15, thick, rounded corners=3pt]
      (4.8,-1) rectangle (8.2,1);

    % three losses inside (stacked vertically inside the right block)
    \foreach \y/\eq in {0.6/${L_\text{ic}(\theta_\text{g})}$,
                        0.0/${L_\text{p}(\theta_\text{g},\theta_\text{p})}$,
                       -0.6/${L_\text{o}(\theta_\text{g})}$} {
      \draw[color=black, rounded corners=3pt, fill=white, thick]
        (5.0, \y-0.2) rectangle (8.0, \y+0.2);
      \node[align=center] at (6.5, \y) {\small \eq};
    }

    % ---- connection from PINO output to Loss block ----
    \draw[-{Latex[length=2mm]}, thick] (4.01,-0.15) -- (4.8,-0.15);

    % ---- external measurement s^(M) goes into the lowest loss ----
    \draw[-{Latex[length=2mm]},thick] (6.5,-1.2) -- (6.5,-0.8);
    \node at (6.7,-1.3) {$\underline{s}^{(M)}$};

    % ---- update theta_g: dashed arrow from Loss back to PINO (top path) ----
    \draw[-{Latex[length=2mm]}, dash pattern=on 4pt off 2pt, thick]
      (4.8,0.1) -- (4.01,0.1);
    \node at (4.4,0.4) {\footnotesize Update ${\theta}_{\text{g}}$};

    % ---- update theta_p: small loop around L_p (middle loss) ----
    \draw[-{Latex[length=2mm]}, dash pattern=on 4pt off 2pt, thick]
      (8.0, 0.15) to[out=30,in=330,looseness=5] (8.0, -0.15);
    \node[align=center] at (8.5, -0.75) {\footnotesize Update\\ \footnotesize ${\theta}_{\text{p}}$};

    % ---- feed (z,t) and s0 down to losses if needed (kept from your scheme) ----
    \draw[-{Latex[length=2mm]}, thick] (0.75,0.1) -- (0.75, 1.2) -- (6.5, 1.2) -- (6.5, 0.8);
\end{tikzpicture}%
}

\newcommand{\timeline}[3][0.15]{%
  \filldraw[gray] (#2, -1.4) circle [radius=1.5pt];
  \node at (#2,-1.7) {\large $\vdots$};
  \filldraw[gray] (#2, -2.2) circle [radius=1.5pt];
  \node at (#2, -2.5) {\large $\vdots$};
  \filldraw[gray] (#2, -3) circle [radius=1.5pt];
  \node at (#2+#1 - 0.1, -3.28) {\small #3};

  % \draw[color=gray]
  %   (#2-#1,-1.3) -- (#2-#1,-3.1)
  %   -- (#2+#1,-3.1)
  %   -- (#2+#1,-1.3) -- (#2-#1,-1.3);
}

% PIDT
\newcommand{\pidt}{
\begin{tikzpicture}
    %Block digital twin
    \node at (4.5, 0.15) {$\hat{s}(z,t)$};
    \draw[color=ForestGreen, fill=ForestGreen!10, rounded corners=3pt, thick] (0.8,-3.55) rectangle (6.2,1.7); \node[align=center] at (1.35, 1.45) {\small PIDT};
    \draw[thick] (0.5, 0) -- (1, 0); \node at (0.15, -2.2) {$(z,t)$};
    \draw[thick] (0.5, -2.2) -- (1, -2.2); \node at (0.15, 0.1) {$\underline{s}^{(0)}$};

    %% Twin model
    \draw[color=RoyalBlue, fill=RoyalBlue!10, rounded corners=3pt, thick] (1,-1.2) rectangle (6,1.2);
    \draw[thick] (1.01,0) -- (2.475,0); \draw[thick] (3.75+0.775,0) -- (5,0);

    \node[rotate=90, align=center] at (1.2+1.04, 0.35) {\small $\underline{\hat{s}}^{(1)}$};
    \node[rotate=90, align=center] at (3.75+1.04, 0.55) {\small $\underline{\hat{s}}^{(M-1)}$};

    \foreach \x/\eq in {1.2/ ${{\beta'_2}^{(1)}, {\gamma'}^{(1)}}$, 2.475/${{\beta'_2}^{(2)}, {\gamma'}^{(2)}}$, 3.75/${{\beta'_2}^{(M-1)}, {\gamma'}^{(M-1)}}$, 5.025/${{\beta'_2}^{(M)}, {\gamma'}^{(M)}}$} {\draw[color=white, rounded corners=3pt, fill=white, thick] (\x, -1) rectangle (\x+0.775, 1); \node[rotate=90, align=center] at (\x+0.3875, 0) {\footnotesize \eq};}

    %%% arrow for output to loss
    \draw[-{Latex[length=2mm]}, thick] (6.7, -2.35) -- (6.7, -5) -- (6.2, -5);
    \node at (6.7, -2.2) {$\hat{s}(z,t)$};

    \filldraw[gray] (1.2+0.775+0.25,0) circle [radius=2pt];
    \filldraw[gray] (3.75+0.775+0.25,0) circle [radius=2pt];
    \filldraw[black] (0.65, 0) circle [radius=2pt];
    \node at (3.5,0) {\normalsize $\cdots$};

    %% Interpolation
    \draw[color=Goldenrod, fill=Goldenrod!10, rounded corners=3pt, thick] (1,-3) rectangle (6,-1.4);

    \draw[Goldenrod, line width=1pt] (2.225, -1.4) -- (1.2+0.775+0.25,-3);
    \draw[Goldenrod, line width=1pt] (4.775, -1.4) -- (3.75+0.775+0.25,-3);
    \draw[Goldenrod, line width=1pt] (3.5, -1.4) -- (3.5,-3);
    \draw[Goldenrod, line width=1pt] (1, -2.2) -- (6, -2.2);

    \timeline{1}{${\underline{s}}^{(0)}$}
    \timeline{2.225}{${\hat{\underline{s}}^{(1)}}$}
    \timeline{3.5}{${\hat{\underline{s}}^{(m)}}$}
    \timeline{4.775}{${\hat{\underline{s}}^{(M-1)}}$}
    \timeline{6}{${\hat{\underline{s}}^{(M)}}$}

    \node at (2.863, -2.2) {\large $\ldots$};
    \node at (4.113, -2.2) {\large $\ldots$};

    \draw [BrickRed, dash pattern=on 4pt off 1pt, thick]  (5.5, -2) circle(4 pt);
    \draw [BrickRed, dash pattern=on 4pt off 2pt, thick] (5.35, -2) -- (1, -2);
    \draw [BrickRed, dash pattern=on 4pt off 2pt, thick] (5.5, -2.15) -- (5.5, -3);
    \node[color=BrickRed] at (1.25, -2.2) {$t$}; \node[color=BrickRed] at (5.3, -2.85) {$z$};
    \filldraw[BrickRed] (5.5, -2) circle [radius=2pt];

    \draw[BrickRed, -{Latex[length=2mm]}, dash pattern=on 4pt off 2pt, thick]
  (5.5, -1.85) to[out=45,in=135,looseness=1] (6.7, -2); \node[color=BrickRed] at (6, -1.5) {\footnotesize Interpolation}; 
  \node at (2.7, -1.63) {\small Intermediate signal matrix};
        
    
    \draw[gray, -{Latex[length=2mm]}, line width=1.2pt] (1.2+0.775+0.25, 0) -- (1.2+0.775+0.25,-1.4); \draw[gray, -{Latex[length=2mm]}, line width=1.2pt] (3.75+0.775+0.25,0) -- (3.75+0.775+0.25,-1.4);    
    %%% Intermediate matrix
    % \foreach \y/\eq in {-1.4-0.2-0.1833, -1.4-2*0.2-0.1833*3, -1.4-3*0.2-0.1833*5} {\draw[fill=white, thick] (3.75+0.775+0.25, \y) circle [radius=0.1666]}
    

    % Loss block
    \draw[color=RedOrange, fill=RedOrange!15, rounded corners=3pt, thick] (0.8,-6) rectangle (6.2,-4);

    %% three losses inside (stacked vertically)
    \foreach \y/\eq in {-5.8/${L_\text{o}(\theta_\text{d})}$,
                        -5.2/${L_\text{p}(\theta_\text{d},\theta_\text{p})}$,
                       -4.6/${L_\text{ic}(\theta_\text{d})}$} {
      \draw[color=black, rounded corners=3pt, fill=white, thick]
        (1, \y) rectangle (6, \y+0.4);
      \node[align=center] at (3.5, \y+0.2) {\small \eq};
    }

    % ---- update theta_p: small loop around L_p (middle loss) ----
    \draw[-{Latex[length=2mm]}, dash pattern=on 4pt off 2pt, thick]
      (1.0, -4.75) to[out=150,in=200,looseness=5] (1.0, -5.15);
    \node[align=center] at (0.5, -5.65) {\footnotesize Update\\ \footnotesize ${\theta}_{\text{p}}$};

    %%% arrow to ic loss and observation loss
    \draw[-{Latex[length=2mm]}, thick] (0.65, 0) -- (0.65, -4.4) -- (1, -4.4);
    \draw[-{Latex[length=2mm]}, thick] (6.7, -5.6) -- (6, -5.6);
    \node at (6.85,-5.8) {$\underline{s}^{(M)}$};

    %%% Backpropogation
    \draw[-{Latex[length=2mm]}, dash pattern=on 4pt off 1pt, thick]
      (3.5, -4) -- (3.5, -3.55);
    \node at (4.2, -3.8) {\footnotesize Update ${\theta}_{\text{d}}$};
\end{tikzpicture}%
}


==> opticameet3_copy.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%                 File: opticameet3.sty               %
%                  Date: 16 June 2022                 %
%                                                     %
%       (c) 2018-2022 Optica Publishing Group         %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\NeedsTeXFormat{LaTeX2e}
\ProvidesPackage{opticameet3}[2022/06/16 LaTeX package for submission to Optica's conferences]

%% packages
\usepackage{cite}
\usepackage{jabbrv}
\RequirePackage{geometry}
\usepackage[dvipsnames]{xcolor}
\usepackage{graphicx}
\usepackage{subcaption}
%% fonts
\usepackage{mathptmx,courier,textcomp}
\usepackage[scaled=.92]{helvet}

\geometry{letterpaper,a4paper,nohead,margin=1in} %% uses geometry.sty
\parindent1em %% em tied to font
\parskip0pc
\linespread{1}
\pagestyle{empty}
\sloppy

%%Title page elements

\newcommand\MEETtitle[1]{\LARGE \bf \hskip2.25pc \parbox{.8\textwidth}{ \noindent%
   \LARGE \bf \begin{center} #1 \end{center}\rm } \vskip.1in \rm\normalsize }

\newcommand\MEETauthor[1]{\hskip2.25pc \parbox{.8\textwidth}{ \noindent%
   \normalsize \bf \begin{center} #1 \end{center}\rm } \vskip-1pc }

\newcommand\MEETaddress[1]{\hskip2.25pc \parbox{.8\textwidth}{ \noindent%
   \footnotesize \it \begin{center} #1 \end{center}\rm }  \normalsize \vskip-.2cm }

\newcommand\MEETemail[1]{\vskip-.3cm \parskip0pc\hskip2.25pc \footnotesize%
   \parbox{.8\textwidth}{\begin{center}\textit{#1}  \end{center} } \normalsize  \vskip-.2cm}



\newcommand\homepage[1]{\vskip-1pt \parskip0pc\hskip2.25pc \footnotesize %% CHANGE 8-3-99
   \parbox{.8\textwidth}{\begin{center}\it \textcolor{blue}{\underline{#1}} \rm \end{center} } \normalsize\vskip-.2cm}

\newcommand\ocis[1]{\vskip-2.75pc \begin{center}\parbox{.8\textwidth}{\footnotesize\bf OCIS codes: \ \rm #1 \hfill} \end{center}\vskip3pt}%

\let\title\MEETtitle
\let\author\MEETauthor
\let\affil\MEETaddress
\let\address\MEETaddress
\let\email\MEETemail
\let\pacs\ocis

%% 29 November, 2018: Allow copyright year to be overridden
\def\@copyrightyear{\number\year}
\newcommand{\copyrightyear}[1]{\def\@copyrightyear{#1}}

\renewenvironment{abstract}%%
{\vskip1pc\noindent\begin{center} \begin{minipage}{.8\textwidth} {\bf Abstract: \ } }
{  \   \vskip1pt\hfil \end{minipage}\end{center}\normalsize\vskip-1.75pc}%

\newenvironment{abstract*}%%
{\vskip1pc\noindent\begin{center} \begin{minipage}{.8\textwidth} {\bf Abstract: \ } }
{ \\  \end{minipage}\end{center}\normalsize\vskip-1.75pc}%

%%Various customizations

\renewcommand\maketitle{\vskip0pt} %%deactivates \maketitle in LaTeX
\def\affiliation{\address}
\def\onlinecite{\citeonline}
%Fig. and Table Labels

\renewcommand\figurename{Fig.}
\def\fps@table{h}%\def\fps@table{!htbp}
\renewcommand\tablename{Table}

%% New caption command
\newcommand\@MaxCapWidth{5.5in}
\setlength\belowcaptionskip{.1in}
\setlength\abovecaptionskip{.15in}
\long\def\@makecaption#1#2{%
  \normalsize
  \vskip\abovecaptionskip
  \sbox\@tempboxa{#1. #2}%
  \ifdim \wd\@tempboxa >\@MaxCapWidth
    \hskip.5in\parbox{5.5in}{#1. #2}
  \else
    \global \@minipagefalse
    \hb@xt@\hsize{\hfil\box\@tempboxa\hfil}%
  \fi
  \vskip\belowcaptionskip\normalsize}

%%References

\renewcommand\refname{\normalsize References \rm}
\setlength\bibindent{.3in}
\renewenvironment{thebibliography}[1]
     {\section*{\refname
        \@mkboth{\MakeUppercase\refname}{\MakeUppercase\refname}}%
      \list{\@arabic\c@enumiv .}
           {\settowidth\labelwidth{.25in}%
            \leftmargin\labelwidth
  \setlength{\parsep}{0pc}
  \setlength{\labelsep}{0.5em}
  \setlength{\itemsep}{0.05pc}%{-0.06in}
  \setlength{\listparindent}{0in}
  \setlength{\itemindent}{0in}
  \setlength{\leftmargin}{.3in}
  \setlength{\rightmargin}{0in}
            \advance\leftmargin\labelsep
            \@openbib@code
            \usecounter{enumiv}%
            \let\p@enumiv\@empty
            \renewcommand\theenumiv{\@arabic\c@enumiv}}%
      \sloppy
      \clubpenalty4000
      \@clubpenalty \clubpenalty
      \widowpenalty4000%
      \sfcode`\.\@m \small}
     {\def\@noitemerr
       {\@latex@warning{Empty `thebibliography' environment}}%
      \endlist \vskip.2in}
\let\@openbib@code\@empty
\newcommand\OPTICAJNLReferences{\thebibliography{}}
\newcommand\OPTICAJNLReflinks{\thebibliography{}}
\newcommand\References{\thebibliography{}}
\newcommand\references{\thebibliography{}}
\let\endOPTICAJNLReferences\endthebibliography
\let\endOPTICAJNLlinks\endthebibliography
\let\endReferences\endthebibliography

%%Section parameters
\renewcommand\@seccntformat[1]{\csname the#1\endcsname.\quad }
\renewcommand\thesubsection{\thesection.\arabic{subsection}}
\renewcommand\thesubsubsection{\thesubsection.\arabic{subsubsection}}

\renewcommand\section{\@startsection {section}{1}{0pt}%
                                   {-2.5ex plus -1ex minus -.2ex}%
                                   {1.3ex plus .2ex}%
                                   {\normalsize\bfseries}}
\renewcommand\subsection{\@startsection{subsection}{2}{0pt}%
                                     {-2.25ex plus -1ex minus -.2ex}%
                                     {1ex plus .2ex}%
                                     {\normalsize\itshape}}
\renewcommand\subsubsection{\@startsection{subsubsection}{3}{0pt}%
                                     {-2.25ex plus -1ex minus -.2ex}%
                                     {1ex plus .2ex}%
                                     {\small\upshape}}

\frenchspacing

\hyphenation {ac-cord-ing
           allow
           back-scat-ter
           back-scat-te-ring
           back-scat-tered
           scat-te-ring
           Based based
           cases
           cen-tered
           changed
           co-incide
           con-cerning
           con-ven-tional
           de-creased
           de-po-lar-iz-ation
           de-tector de-tectors
           de-vi-ation
           dis-cussion
           dis-tribu-tion
           dis-tribu-tions
           dis-trib-ute
           dis-trib-uted
           Ehhalt
           extinc-tion
           found
           Geest-hacht
           ground
           Hink-ley
           il-lus-trated
           il-lus-trate
           Intro-ducing
           Klap-heck
           lati-tude
           measure-ment
           measure-ments
           meas-ured
           measuring
           mixing
           north-east
           orig-inated
           op-er-ating
           out-flow
           pres-ence
           primary
           rather
           rela-tive
           sig-nal
           sig-nals
           solid
           tem-pera-ture
           Tem-pera-ture
           trans-ported
           tropo-pause
           Tropo-pause
           tropo-sphere
           Tropo-sphere
           tube
           tubes
           Values
           varies
           Weather}

\def\opex{ Opt.\ Express }
\def\ao{ Appl.\  Opt.\ }
\def\ap{ Appl.\  Phys.\ }
\def\apa{ Appl.\  Phys.\ A }
\def\apb{ Appl.\  Phys.\ B }
\def\apl{ Appl.\ Phys.\ Lett.\ }
\def\apj{ Astrophys.\ J.\ }
\def\bell{ Bell Syst.\ Tech.\ J.\ }
\def\jqe{ IEEE J.\ Quantum Electron.\ }
\def\assp{ IEEE Trans.\ Acoust.\ Speech Signal Process.\ }
\def\aprop{ IEEE Trans.\ Antennas Propag.\ }
\def\mtt{ IEEE Trans.\ Microwave Theory Tech.\ }
\def\iovs{ Invest.\ Ophthalmol.\ Visual\ Sci.\ }
\def\jcp{ J.\ Chem.\ Phys.\ }
\def\jmo{ J.\ Mod.\ Opt.\ }
\def\jon{J.\ Opt.\ Netw.\ }
\def\josa{ J.\ Opt.\ Soc.\ Am.\ }
\def\josaa{ J.\ Opt.\ Soc.\ Am.\ A }
\def\josab{ J.\ Opt.\ Soc.\ Am.\ B }
\def\jpp{ J.\ Phys.\ (Paris) }
\def\nat{ Nature (London) }
\def\oc{ Opt.\ Commun.\ }
\def\ol{ Opt.\ Lett.\ }
\def\pl{ Phys.\ Lett.\ }
\def\pra{ Phys.\ Rev.\ A }
\def\prb{ Phys.\ Rev.\ B }
\def\prc{ Phys.\ Rev.\ C }
\def\prd{ Phys.\ Rev.\ D }
\def\pre{ Phys.\ Rev.\ E }
\def\prl{ Phys.\ Rev.\ Lett.\ }
\def\rmp{ Rev.\ Mod.\ Phys.\ }
\def\pspie{ Proc.\ SPIE\ }
\def\sjqe{ Sov.\ J.\ Quantum Electron.\ }
\def\vr{ Vision Res.\ }
\def\cleo{ {\it Conference on Lasers and Electro-Optics }}
\def\assl{ {\it Advanced Solid State Lasers }}
\def\tops{ Trends in Optics and Photonics }

%% end opticameet3.sty

